Malware MultiVerse: From Automatic Logic Bomb Identification to Automatic Patching and Tracing

Malware and other suspicious software often hide behaviors and components behind logic bombs and context-sensitive execution paths. Uncovering these is essential to react against modern threats, but current solutions are not ready to detect these paths in a completely automated manner. To bridge this gap, we propose the Malware Multiverse (MalVerse), a solution able to inspect multiple execution paths via symbolic execution aiming to discover function inputs and returns that trigger malicious behaviors. MalVerse automatically patches the context-sensitive functions with the identified symbolic values to allow the software execution in a traditional sandbox. We implemented MalVerse on top of angr and evaluated it with a set of Linux and Windows evasive samples. We found that MalVerse was able to generate automatic patches for the most common evasion techniques (e.g., ptrace checks).

==> Sections/app.tex <==
\section{Automatic identification Code Sample}
\label{app:code:sample}

Code~\ref{code:sample1} shows an example of
an \angr script that automatically decompiles
the function by concretizing a symbolic value.

\begin{lstlisting}[frame=single,label=code:sample1, caption={\textbf{Angr Script Example.} Automatic Identification and Decompilation.}]
# Project
p = angr.Project(sys.argv[1], load_options={"auto_load_libs":False})
# Normalized for decompilation
cfg = p.analyses.CFGFast(normalize=True)
# From begining
state = p.factory.entry_state()
sm = p.factory.simulation_manager(state)
# Until find the target
func = cfg.functions.get('target_function_name')
found = sm.explore(find=func.addr)
# get first decision point
decision_func = found.found[0].history.simprocs.hardcopy[0]
# Update state for the current one
decision_func.set_state(found.found[0])
# get handler to this func in the original cfg
cfg_func = cfg.functions.get(decision_func.name)
# Original decompilation
dec = p.analyses.Decompiler(cfg_func) 
dec.codegen.text
# Concretized decompilation
dec = p.analyses.Decompiler(cfg_func,concrete_values=decision_func)
dec.codegen.text
\end{lstlisting}

\section{AV Detection of DDoS Samples}
\label{app:transfer}

Table~\ref{sec:xarcen} shows the MD5 hashes of the samples identified as similar by \tool and the associated detection labels assigned by the Kaspersky AV,

\begin{table*}[!htpb]
\caption{\textbf{DDoS Samples.} AV-assigned labels.}
\label{sec:xarcen}
\centering
\begin{tabular}{cc}
\hline
\textbf{Hash (MD5)} & \textbf{Label} \\ \hline
47180153336a9f3c0a8b93fc922216705690f36fc7b25148e44d3a1be4e1a32b &   HEUR:Trojan-DDoS.Linux.Xarcen.d \\
83ed6adc167fd73f21ca6ae03e1d214ec71cf5bb153c7cbdbed35a4e4c994370  &    Undetected                      \\
6855d4307e775de546d00b2357299e5f85c18ab1d79962b2bbb9f917758cfad7   &   HEUR:Trojan-DDoS.Linux.Xarcen.d \\
8ed19e85a5cd5fb0106e4066523fed1f8b100ef0ad557198fba10749cafabf1e  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
0636d8749ecb285c293dc533c9b7690ba17ac7902488bf39164129a12d54c1c3  &     Undetected                      \\
3025a698a0ee802e0a667b2288578ee0e15191e2320c78997bb9a8ad3e32c473  &     Trojan-DDoS.Linux.Xarcen.c      \\
5776ea75b5f8faa6e4d8ac7000ed35c282d4904fb820c2b7c5df10fa8adaaa55  &    HEUR:Trojan-DDoS.Linux.Xarcen.a \\
891b01d92d0366fbb4af44135cfb9b4b9f9d2b28cc052f70cb9724ef30545608  &     Undetected                      \\
a6b8d218bfa051b3234977290ad6c9af6c3ea7dcf26b643b381f8876f12e7d68  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
ea520d2eb6a7ee8e1caad62bd3e81e6821e63202076cc84c63d7bdff66d64565  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
7aa8eab2f01783bfe9bb7d8e051baebf563629645d73b2af42022d28a8143179   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
3bb61c0ad19495ae554363823eb83657b403c3aacdf9cddb9b111c2c4321a6da  &     Undetected                      \\
94b59b4761147519fecf662cecba7219ac2f70682ae02685081a181758cb705f   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
3b69274ed57f87c9865c8bb6eaf456bcc64d7141def3abfc1051ecd94061d0a3  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
2409fb21fe377f7e12dda392f26d7c93b7715239169d362dd907fe499ab38ee9   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
e8cb63cc050c952c1168965f597105a128b56114835eb7d40bdec964a0e243dc  &      HEUR:Trojan-DDoS.Linux.Xarcen.a \\
878a1ae13649b3943216a5b1aa90f0d2a71d1550393e8a03cffc4f0cb3cd5431  &     Undetected                      \\
c46126e4c3788efa5e62638b807e472f58e9e1b2636fd2473105794bd32cfe12  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
ce46658b3ec80b2d25eac5b629b488f5808cce2da8683daad58bb23204bb0aad  &     HEUR:Trojan-DDoS.Linux.Agent.g  \\
6c3d6e79cd6e09f169c188010751d03efa9dfa9f31d4abf7ef7780be255d337a   &   HEUR:Trojan-DDoS.Linux.Agent.g  \\
0ba0a4fcc2faaf2448a6ef9dde8c76a228293e60f1587531938c25d46407f6a4  &     Trojan-DDoS.Linux.Xarcen.c      \\
1e90557835fefc446de6b2f9b431065fc3ad0dec881b924f02d9a16336d446b0  &     Undetected                      \\
4ddcf98edfa5691d725c07e2144edd3c407d5fcfc92c485a78108fbcae245658  &     Trojan-DDoS.Linux.Xarcen.c      \\
8c8aad32ee169ba6240874920253b3250f6785bc19c42c304771979ed43ec0af   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
8569e3183041e673f2c6f281aad519d8557abfd7650abac491991ad0775b18f4   &   Trojan-DDoS.Linux.Xarcen.c      \\
4240e265ad237382e5a2c22f65f022775c07463e5309439d226c2cc1f852624b   &   HEUR:Trojan-DDoS.Linux.Agent.g  \\
2eeb12940749e9aa138dd91bb343d8e4f5822beda9d378022b32714c1ea10fdb  &     Undetected                      \\
af4323d7f8b4626eaa5e110a3bfb59f1dd2b555cd7a5b801b667af80e306ff74   &   HEUR:Trojan-DDoS.Linux.Agent.g  \\
9c79670d65ffd317d7f1a0ca75e4870720a0321f8634f7ec7fe2385e28222c26  &     Undetected                      \\
8c64fe221e6f8fe2ec785b0fc5b1c6250ca3ef26f5dcfae65b98d38f125baca6  &     HEUR:Trojan-DDoS.Linux.Agent.g  \\
12e004b5ad8f41f489ff3bc4d2384b99284de97d4f1559c4c64a7921cd8a9a1e  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
d8ebf75697902e883006fc46410558d98c667bc50ebf374d2acd5cc3bfcdc2ff  &     Undetected                      \\
e55b3df36841269015aec43faef1dc9a1364f430ebbdee43c5bc9b68245ba076  &     HEUR:Trojan-DDoS.Linux.Xarcen.d \\
dae1034c283bcabc20d9c71179f4cf7b14594946cc8b22c7edf9e1bf1815828e  &     Undetected                      \\
142e14d7872cbd783246d3be0396f3eb3c9fbd2c30d571ff3bd7769e00c08fcd  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
d1b26fc704cc236cfcc340b93adfa221611bcd040a4907206fc50e8749d189c6  &     Undetected                      \\
24b3229bc8afe04792bd2cef450f049aad282be5d1112819cf26efdd1747ff7c  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
2815c35a00c6abadc22aa61b888cb144bc51458d08196794f15d06851d185b1d  &     Undetected                      \\
3537edea0998560769b90739d9007611806ebc779a8cf8f730f822f50e383a4b  &     HEUR:Trojan-DDoS.Linux.Xarcen.d \\
3d10efc61537b2a16e9552aba706017c18afce95da394bcca0c0de4b75f08d02   &   Trojan-DDoS.Linux.Xarcen.c      \\
02ab39d5ef83ffd09e3774a67b783bfa345505d3cb86694c5b0f0c94980e5ae8   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
be6e4a44e83bb1efde29ec27214c0b66ef174dd1892166aac47b332c4f3162f9  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
965ac4ef69daaca3f2797bf97b0b480de1a002d3d3a055613c364806d7826e34   &   HEUR:Trojan-DDoS.Linux.Xarcen.a \\
98d9130bc6a6b7f83809fcf5e09bc72cde3820e933ac48b58c37ecdee3f705b8  &     HEUR:Trojan-DDoS.Linux.Xarcen.a \\
5d6c8c82ed6d218478b6a6cb9e9808c5248de52eff4eaadabb94766c3c8e8e23  &     Undetected                      \\
c880a315a26033b2117bf4e99630c099e98767a453ae14eac00f16b9846e372a  &    HEUR:Trojan-DDoS.Linux.Xarcen.a \\
27877a0aa3f7edecdb3c7dace40cb5f135a4ab0bf2b1d73489ab93c170311b73  &     Undetected                      \\
8c459a7cf1337bca62c256717273bb49c1166b05c97b5afcd5b04932beb33b97   &   Undetected                      \\
5bb5f065655228ed1754e69be308aff634dadb9eca6d223fa78db08bb2203f4b   &   Trojan-DDoS.Linux.Xarcen.c      \\
eb0c0587cf20c81921b7b6d174177ef8b11133bb65a760d9016fbdce917a2ee6  &     Trojan-DDoS.Linux.Xarcen.c      \\
67118ecdec90a8133d6a02b00c03d1c0d83ebbb0428fadc20bf08c14451a9e26  &     Undetected                      \\ \hline
\end{tabular}
\end{table*}
